Meta-Monomorphizing Specializations

Achieving zero-cost specialization remains a fundamental challenge in programming language and compiler design. It often necessitates trade-offs between expressive power and type system soundness, as the interaction between conditional compilation and static dispatch can easily lead to unforeseen coherence violations and increased complexity in the formal model. This paper introduces meta-monomorphizing specializations, a novel framework that achieves specialization by repurposing monomorphization through compile-time metaprogramming. Instead of modifying the host compiler, our approach generates meta-monomorphized traits and implementations that encode specialization constraints directly into the type structure, enabling deterministic, coherent dispatch without overlapping instances. We formalize this method for first-order, predicate-based, and higher-ranked polymorphic specialization, also in presence of lifetime parameters. Our evaluation, based on a Rust implementation using only existing macro facilities, demonstrates that meta-monomorphization enables expressive specialization patterns while maintaining full compatibility with standard optimization pipelines. We show that specialization can be realized as a disciplined metaprogramming layer, offering a practical, language-agnostic path to high-performance abstraction. A comprehensive study of public Rust codebases further validates our approach, revealing numerous workarounds that meta-monomorphization can eliminate, leading to more idiomatic and efficient code. An empirical evaluation on 16 micro-benchmarks confirms that compile-time specialization matches or outperforms runtime TypeId-based dispatch, and demonstrates expressiveness gains on patterns -- such as lifetime-based dispatch, higher-ranked types, compound predicates, and wildcard matching -- that runtime dispatch structurally cannot express.

==> fix_star.tex <==
\ExplSyntaxOn
\cs_new_eq:NN \Repeat \prg_replicate:nn
\ExplSyntaxOff
\makeatletter
\ifdoubleblind\else%The default behavior is to disable title footnotes for doubleblind reviews (the edit will fail if applied with the doubleblind option)
    \patchcmd{\tnotetext}{\ifcase\c@tnote\or$\star$\or$\star\star$\fi}{\Repeat{\the\c@tnote}{\tnotemarksymbol}}{}{\@latex@error{Failed to patch \string\tnotetext}}
    \patchcmd{\tnotemark}{\expandafter\ifcase\elsRef{\mytmark}\or$^{\star}$\or$^{,\star\star}$\fi}{\textsuperscript{\expandafter\ifnum\elsRef{\mytmark}>1,\fi\expandafter\Repeat\expandafter{\elsRef{\mytmark}}{\tnotemarksymbol}}}{}{\@latex@error{Failed to patch \string\tnotemark}}%
\fi
\makeatother
\newcommand{\tnotemarksymbol}{\dag}


==> tables/dataset.tex <==
{
% \begin{landscape}
    \rowcolors{2}{gray!10}{white}
	\footnotesize % \tiny
    \begin{longtable}{
            % @{\extracolsep{\fill}}
            >{\raggedright\arraybackslash}m{0.25cm} |
            >{\raggedright\arraybackslash}m{2.5cm}
            >{\centering\arraybackslash}m{1.2cm}
            >{\centering\arraybackslash}m{2cm}
            >{\centering\arraybackslash}m{2cm}
            >{\centering\arraybackslash}m{1.25cm}
            >{\centering\arraybackslash}m{1.25cm}
    }
        \toprule
        \rowcolor{white}
        & \textbf{Project Name} & \textbf{Stars} & \textbf{Dependencies} & \textbf{Downloads} & \textbf{Functions} & \textbf{Traits } \\
		\midrule
		\endfirsthead

		\toprule
        \rowcolor{white}
         & \textbf{Project Name} & \textbf{Stars} & \textbf{Dependencies} & \textbf{Downloads} & \textbf{Functions} & \textbf{Traits } \\
		\midrule
		\endhead


		\midrule
        \rowcolor{white}
		\multicolumn{7}{r}{\textit{Continued on next page}} \\
		\midrule
		\endfoot

		\bottomrule
        \rowcolor{white}
        \multicolumn{7}{c}{ } \\
        \caption{Dataset of analyzed Rust projects with their GitHub stars, number of dependent crates, total downloads from \texttt{crates.io}, number of functions, and number of traits.}
        \label{table:dataset}
		\endlastfoot

1      & \href{https://github.com/dtolnay/syn}{syn}                                   & 3215    & 12774  & 1169638606  & 11140    & 129      \\
2      & \href{https://github.com/rust-lang/hashbrown}{hashbrown}                     & 2799    & 1433   & 948648240   & 727      & 34       \\
3    	 & \href{https://github.com/bitflags/bitflags}{bitflags}                        & 1068    & 3583   & 871628003   & 161      & 26       \\
4      & \href{https://github.com/dtolnay/proc-macro2}{proc-macro2}                   & 880     & 10815  & 806768972   & 460      & 16       \\
5      & \href{https://github.com/dtolnay/quote}{quote}                               & 1485    & 12614  & 788009739   & 395      & 32       \\
6      & \href{https://github.com/marshallpierce/rust-base64}{base64}                 & 697     & 7686   & 786716305   & 84       & 14       \\
7      & \href{https://github.com/rust-lang/libc}{libc}                               & 2363    & 8291   & 784673557   & 583      & 10       \\
8      & \href{https://github.com/rust-random/getrandom}{getrandom}                   & 466     & 1755   & 748944236   & 38       & 3        \\
9      & \href{https://github.com/rust-random/rand}{rand}                             & 1934    & 21883  & 743653059   & 598      & 50       \\
10     & \href{https://github.com/indexmap-rs/indexmap}{indexmap}                     & 2221    & 3415   & 705015407   & 931      & 42       \\
11     & \href{https://github.com/rust-lang/cfg-if}{cfg-if}                           & 613     & 2364   & 702351853   & 0        & 0        \\
12     & \href{https://github.com/serde-rs/serde}{serde}                              & 10133   & 61896  & 702283491   & 3141     & 71       \\
13     & \href{https://github.com/rust-itertools/itertools}{itertools}                & 3033    & 7169   & 702204937   & 865      & 33       \\
14     & \href{https://github.com/cuviper/autocfg}{autocfg}                           & 105     & 69     & 649484539   & 50       & 2        \\
15     & \href{https://github.com/BurntSushi/memchr}{memchr}                          & 1261    & 985    & 640677127   & 367      & 9        \\
16     & \href{https://github.com/dtolnay/itoa}{itoa}                                 & 349     & 437    & 635152777   & 18       & 3        \\
17     & \href{https://github.com/serde-rs/json}{json}                                & 5373    & 539    & 616768830   & 1432     & 49       \\
18     & \href{https://github.com/dtolnay/thiserror}{thiserror}                       & 5199    & 29908  & 613253638   & 188      & 21       \\
19     & \href{https://github.com/dtolnay/unicode-ident}{unicode-ident}               & 103     & 83     & 612334907   & 15       & 1        \\
20     & \href{https://github.com/matklad/once_cell}{once\_cell}                      & 2039    & 6860   & 609099441   & 106      & 8        \\
21     & \href{https://github.com/rust-lang/log}{log}                                 & 2443    & 24032  & 607963553   & 77       & 7        \\
22     & \href{https://github.com/withoutboats/heck}{heck}                            & 569     & 1175   & 606082034   & 23       & 12       \\
23     & \href{https://github.com/rust-lang/cc-rs}{cc}                                & 2054    & 2868   & 578138896   & 517      & 20       \\
24     & \href{https://github.com/rust-lang/regex}{regex}                             & 3830    & 14186  & 576863005   & 3597     & 89       \\
25     & \href{https://github.com/dtolnay/ryu}{ryu}                                   & 668     & 217    & 575741455   & 43       & 3        \\
26     & \href{https://github.com/clap-rs/clap}{clap}                                 & 15713   & 26880  & 565116789   & 1730     & 73       \\
27     & \href{https://github.com/aho-corasick}{aho-corasick}                         & 1155    & 241    & 564252056   & 699      & 26       \\
28     & \href{https://github.com/servo/rust-smallvec}{smallvec}                      & 1557    & 2206   & 560988870   & 174      & 35       \\
29     & \href{https://github.com/rapidfuzz/strsim-rs}{strsim}                        & 457     & 327    & 539207767   & 29       & 3        \\
30     & \href{https://github.com/Amanieu/parking_lot}{parking\_lot}                  & 3160    & 4078   & 534825577   & 363      & 35       \\
31     & \href{https://github.com/rust-lang-nursery/lazy-static.rs}{lazy\_static}     & 2022    & 10657  & 524896258   & 2        & 0        \\
32     & \href{https://github.com/rust-num/num-traits}{num-traits}                    & 886     & 5577   & 516997081   & 2585     & 47       \\
33     & \href{https://github.com/rust-lang/socket2}{socket2}                         & 807     & 606    & 511596457   & 350      & 12       \\
34     & \href{https://github.com/dtolnay/semver}{semver}                             & 647     & 2040   & 490095892   & 87       & 14       \\
35     & \href{https://github.com/RustCrypto/traits}{digest}                          & 690     & 924    & 490088430   & 1142     & 164      \\
36     & \href{https://github.com/rayon-rs/either}{either}                            & 540     & 1196   & 489778929   & 132      & 19       \\
37     & \href{https://github.com/SergioBenitez/version_check}{version\_check}        & 53      & 159    & 489739708   & 38       & 2        \\
38     & \href{https://github.com/bytecodealliance/rustix}{rustix}                    & 1808    & 326    & 489109186   & 1809     & 39       \\
39     & \href{https://github.com/tokio-rs/bytes}{bytes}                              & 2124    & 8941   & 476345608   & 695      & 34       \\
40     & \href{https://github.com/time-rs/time}{time}                                 & 1242    & 3768   & 474012695   & 1558     & 60       \\
41     & \href{https://github.com/servo/rust-url}{url}                                & 1485    & 8985   & 440112102   & 365      & 34       \\
42     & \href{https://github.com/toml-rs/toml}{toml}                                 & 930     & 7698   & 419494766   & 2233     & 122      \\
43     & \href{https://github.com/rust-lang/futures-rs}{futures}                      & 5757    & 15877  & 387648094   & 2313     & 126      \\
44     & \href{https://github.com/rust-lang/glob}{glob}                               & 564     & 2294   & 298438955   & 32       & 7        \\
45     & \href{https://github.com/quickwit-oss/tantivy}{tantivy}                      & 13983   & 119    & 8443224     & 3871     & 150      \\
46     & \href{https://github.com/tauri-apps/tauri}{tauri}                            & 98798   & 326    & 8149533     & 4898     & 196      \\
47     & \href{https://github.com/pola-rs/polars}{polars}                             & 36050   & 368    & 6552820     & 43805    & 1476     \\
48     & \href{https://github.com/rust-lang/cargo}{cargo}                             & 14225   & 125    & 5437801     & 4441     & 108      \\
49     & \href{https://github.com/sharkdp/bat}{bat}                                   & 55795   & 76     & 2625346     & 356      & 16       \\
50     & \href{https://github.com/BurntSushi/ripgrep}{ripgrep}                        & 57234   & 1      & 1279887     & 2096     & 66       \\
51     & \href{https://github.com/cloudflare/quiche}{quiche}                          & 10869   & 21     & 1239916     & 2607     & 110      \\
52     & \href{https://github.com/influxdata/influxdb}{influxdb}                      & 30797   & 25     & 443557      & 3547     & 212      \\
53     & \href{https://github.com/typst/typst}{typst}                                 & 47949   & 71     & 311285      & 7260     & 233      \\
54     & \href{https://github.com/alacritty/alacritty}{alacritty}                     & 61003   & 0      & 242002      & 2710     & 72       \\
55     & \href{https://github.com/helix-editor/helix}{helix}                          & 41235   & 0      & 117928      & 3080     & 116      \\
56     & \href{https://github.com/Nukesor/pueue}{pueue}                               & 5903    & 0      & 106705      & 389      & 24       \\
57     & \href{https://github.com/GitoxideLabs/gitoxide}{gitoxide}                    & 10519   & 0      & 104688      & 7148     & 484      \\
58     & \href{https://github.com/EmbarkStudios/texture-synthesis}{texture-synthesis} & 1793    & 1      & 69074       & 166      & 10       \\
59     & \href{https://github.com/n0-computer/sendme}{sendme}                         & 832     & 0      & 31181       & 74       & 7        \\
60     & \href{https://github.com/unionlabs/union}{union}                             & 74491   & 1      & 16742       & 29581    & 1050     \\
61     & \href{https://github.com/zed-industries/zed}{zed}                            & 69551   & N/A    & N/A         & 54980    & 1674     \\
62     & \href{https://github.com/charliermarsh/ruff}{ruff}                           & 43777   & N/A    & N/A         & 25887    & 640      \\
63     & \href{https://github.com/juspay/hyperswitch}{hyperswitch}                    & 39130   & N/A    & N/A         & 32172    & 826      \\
64     & \href{https://github.com/lapce/lapce}{lapce}                                 & 37601   & N/A    & N/A         & 1797     & 62       \\
65     & \href{https://github.com/nushell/nushell}{nushell}                           & 37226   & N/A    & N/A         & 10592    & 330      \\
        % \hline

   \end{longtable} 
}

% \begin{table*}[tbh!]
%   \caption{}%
%   \label{table:results}
%   \centering
%   % \scriptsize
%   % \resizebox{\textwidth}{!}{%
%   \resizebox{\textwidth}{!}{%
%   % \begin{tabular}{>{\ttfamily}lrrrrr}
%   \begin{tabular}{c||lccccc}
%     \toprule
%     \multicolumn{1}{>{\bfseries\centering}p{0.15cm}}{} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{Project Name} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{GitHub Stars} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{Dependency} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{Downloads} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{\# Functions} &
%     \multicolumn{1}{>{\bfseries\centering}p{1cm}}{\# Traits } \\\midrule
%
% 1      & \href{https://github.com/dtolnay/syn}{syn}                                   & 3215    & 12774  & 1169638606  & 11140    & 129      \\
% 2      & \href{https://github.com/rust-lang/hashbrown}{hashbrown}                     & 2799    & 1433   & 948648240   & 727      & 34       \\
% 3    	 & \href{https://github.com/bitflags/bitflags}{bitflags}                        & 1068    & 3583   & 871628003   & 161      & 26       \\
% 4      & \href{https://github.com/dtolnay/proc-macro2}{proc-macro2}                   & 880     & 10815  & 806768972   & 460      & 16       \\
% 5      & \href{https://github.com/dtolnay/quote}{quote}                               & 1485    & 12614  & 788009739   & 395      & 32       \\
% 6      & \href{https://github.com/marshallpierce/rust-base64}{base64}                 & 697     & 7686   & 786716305   & 84       & 14       \\
% 7      & \href{https://github.com/rust-lang/libc}{libc}                               & 2363    & 8291   & 784673557   & 583      & 10       \\
% 8      & \href{https://github.com/rust-random/getrandom}{getrandom}                   & 466     & 1755   & 748944236   & 38       & 3        \\
% 9      & \href{https://github.com/rust-random/rand}{rand}                             & 1934    & 21883  & 743653059   & 598      & 50       \\
% 10     & \href{https://github.com/indexmap-rs/indexmap}{indexmap}                     & 2221    & 3415   & 705015407   & 931      & 42       \\
% 11     & \href{https://github.com/rust-lang/cfg-if}{cfg-if}                           & 613     & 2364   & 702351853   & 0        & 0        \\
% 12     & \href{https://github.com/serde-rs/serde}{serde}                              & 10133   & 61896  & 702283491   & 3141     & 71       \\
% 13     & \href{https://github.com/rust-itertools/itertools}{itertools}                & 3033    & 7169   & 702204937   & 865      & 33       \\
% 14     & \href{https://github.com/cuviper/autocfg}{autocfg}                           & 105     & 69     & 649484539   & 50       & 2        \\
% 15     & \href{https://github.com/BurntSushi/memchr}{memchr}                          & 1261    & 985    & 640677127   & 367      & 9        \\
% 16     & \href{https://github.com/dtolnay/itoa}{itoa}                                 & 349     & 437    & 635152777   & 18       & 3        \\
% 17     & \href{https://github.com/serde-rs/json}{json}                                & 5373    & 539    & 616768830   & 1432     & 49       \\
% 18     & \href{https://github.com/dtolnay/thiserror}{thiserror}                       & 5199    & 29908  & 613253638   & 188      & 21       \\
% 19     & \href{https://github.com/dtolnay/unicode-ident}{unicode-ident}               & 103     & 83     & 612334907   & 15       & 1        \\
% 20     & \href{https://github.com/matklad/once_cell}{once\_cell}                      & 2039    & 6860   & 609099441   & 106      & 8        \\
% 21     & \href{https://github.com/rust-lang/log}{log}                                 & 2443    & 24032  & 607963553   & 77       & 7        \\
% 22     & \href{https://github.com/withoutboats/heck}{heck}                            & 569     & 1175   & 606082034   & 23       & 12       \\
% 23     & \href{https://github.com/rust-lang/cc-rs}{cc}                                & 2054    & 2868   & 578138896   & 517      & 20       \\
% 24     & \href{https://github.com/rust-lang/regex}{regex}                             & 3830    & 14186  & 576863005   & 3597     & 89       \\
% 25     & \href{https://github.com/dtolnay/ryu}{ryu}                                   & 668     & 217    & 575741455   & 43       & 3        \\
% 26     & \href{https://github.com/clap-rs/clap}{clap}                                 & 15713   & 26880  & 565116789   & 1730     & 73       \\
% 27     & \href{https://github.com/aho-corasick}{aho-corasick}                         & 1155    & 241    & 564252056   & 699      & 26       \\
% 28     & \href{https://github.com/servo/rust-smallvec}{smallvec}                      & 1557    & 2206   & 560988870   & 174      & 35       \\
% 29     & \href{https://github.com/rapidfuzz/strsim-rs}{strsim}                        & 457     & 327    & 539207767   & 29       & 3        \\
% 30     & \href{https://github.com/Amanieu/parking_lot}{parking\_lot}                  & 3160    & 4078   & 534825577   & 363      & 35       \\
% 31     & \href{https://github.com/rust-lang-nursery/lazy-static.rs}{lazy\_static}     & 2022    & 10657  & 524896258   & 2        & 0        \\
% 32     & \href{https://github.com/rust-num/num-traits}{num-traits}                    & 886     & 5577   & 516997081   & 2585     & 47       \\
% 33     & \href{https://github.com/rust-lang/socket2}{socket2}                         & 807     & 606    & 511596457   & 350      & 12       \\
% 34     & \href{https://github.com/dtolnay/semver}{semver}                             & 647     & 2040   & 490095892   & 87       & 14       \\
% 35     & \href{https://github.com/RustCrypto/traits}{digest}                          & 690     & 924    & 490088430   & 1142     & 164      \\
% 36     & \href{https://github.com/rayon-rs/either}{either}                            & 540     & 1196   & 489778929   & 132      & 19       \\
% 37     & \href{https://github.com/SergioBenitez/version_check}{version\_check}        & 53      & 159    & 489739708   & 38       & 2        \\
% 38     & \href{https://github.com/bytecodealliance/rustix}{rustix}                    & 1808    & 326    & 489109186   & 1809     & 39       \\
% 39     & \href{https://github.com/tokio-rs/bytes}{bytes}                              & 2124    & 8941   & 476345608   & 695      & 34       \\
% 40     & \href{https://github.com/time-rs/time}{time}                                 & 1242    & 3768   & 474012695   & 1558     & 60       \\
% 41     & \href{https://github.com/servo/rust-url}{url}                                & 1485    & 8985   & 440112102   & 365      & 34       \\
% 42     & \href{https://github.com/toml-rs/toml}{toml}                                 & 930     & 7698   & 419494766   & 2233     & 122      \\
% 43     & \href{https://github.com/rust-lang/futures-rs}{futures}                      & 5757    & 15877  & 387648094   & 2313     & 126      \\
% 44     & \href{https://github.com/rust-lang/glob}{glob}                               & 564     & 2294   & 298438955   & 32       & 7        \\
% 45     & \href{https://github.com/quickwit-oss/tantivy}{tantivy}                      & 13983   & 119    & 8443224     & 3871     & 150      \\
% 46     & \href{https://github.com/tauri-apps/tauri}{tauri}                            & 98798   & 326    & 8149533     & 4898     & 196      \\
% 47     & \href{https://github.com/pola-rs/polars}{polars}                             & 36050   & 368    & 6552820     & 43805    & 1476     \\
% 48     & \href{https://github.com/rust-lang/cargo}{cargo}                             & 14225   & 125    & 5437801     & 4441     & 108      \\
% 49     & \href{https://github.com/sharkdp/bat}{bat}                                   & 55795   & 76     & 2625346     & 356      & 16       \\
% 50     & \href{https://github.com/BurntSushi/ripgrep}{ripgrep}                        & 57234   & 1      & 1279887     & 2096     & 66       \\
% 51     & \href{https://github.com/cloudflare/quiche}{quiche}                          & 10869   & 21     & 1239916     & 2607     & 110      \\
% 52     & \href{https://github.com/influxdata/influxdb}{influxdb}                      & 30797   & 25     & 443557      & 3547     & 212      \\
% 53     & \href{https://github.com/typst/typst}{typst}                                 & 47949   & 71     & 311285      & 7260     & 233      \\
% 54     & \href{https://github.com/alacritty/alacritty}{alacritty}                     & 61003   & 0      & 242002      & 2710     & 72       \\
% 55     & \href{https://github.com/helix-editor/helix}{helix}                          & 41235   & 0      & 117928      & 3080     & 116      \\
% 56     & \href{https://github.com/Nukesor/pueue}{pueue}                               & 5903    & 0      & 106705      & 389      & 24       \\
% 57     & \href{https://github.com/GitoxideLabs/gitoxide}{gitoxide}                    & 10519   & 0      & 104688      & 7148     & 484      \\
% 58     & \href{https://github.com/EmbarkStudios/texture-synthesis}{texture-synthesis} & 1793    & 1      & 69074       & 166      & 10       \\
% 59     & \href{https://github.com/n0-computer/sendme}{sendme}                         & 832     & 0      & 31181       & 74       & 7        \\
% 60     & \href{https://github.com/unionlabs/union}{union}                             & 74491   & 1      & 16742       & 29581    & 1050     \\
% 61     & \href{https://github.com/zed-industries/zed}{zed}                            & 69551   & N/A    & N/A         & 54980    & 1674     \\
% 62     & \href{https://github.com/charliermarsh/ruff}{ruff}                           & 43777   & N/A    & N/A         & 25887    & 640      \\
% 63     & \href{https://github.com/juspay/hyperswitch}{hyperswitch}                    & 39130   & N/A    & N/A         & 32172    & 826      \\
% 64     & \href{https://github.com/lapce/lapce}{lapce}                                 & 37601   & N/A    & N/A         & 1797     & 62       \\
% 65     & \href{https://github.com/nushell/nushell}{nushell}                           & 37226   & N/A    & N/A         & 10592    & 330      \\
%
%
%
%     % \midrule
%
%     \bottomrule
%
%   \end{tabular}
%   }
% \end{table*}


==> tables/results-old.tex <==
{
% \begin{landscape}
    \rowcolors{2}{gray!10}{white}
	\footnotesize % \tiny
    \begin{longtable}{
            % @{\extracolsep{\fill}}
            >{\raggedright\arraybackslash}m{0.25cm} |
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.75cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.8cm} ||
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.75cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.8cm}
    }
        \toprule
        \rowcolor{white}
        \multicolumn{7}{c}{\textbf{Threshold 90\%}} & \multicolumn{6}{c}{\textbf{Threshold 99\%}}\\
         & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} \\
		\midrule
		\endfirsthead

		\toprule
        \rowcolor{white}
        \multicolumn{7}{c}{\textbf{Threshold 90\%}} & \multicolumn{6}{c}{\textbf{Threshold 99\%}}\\
         & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} \\
		\midrule
		\endhead


		\midrule
        \rowcolor{white}
		\multicolumn{13}{r}{\textit{Continued on next page}} \\
		\midrule
		\endfoot

		\bottomrule
        \rowcolor{white}
        \multicolumn{13}{c}{ } \\
        \caption{TODO}
        \label{tab:results}
		\endlastfoot

1      & 167.12     & 200        & 2394     & 21.5\%   					& 36       & 27.9\% 							& 200.97     & 181        & 1313     & 11.8\%							& 30       & 23.3\% 							\\
2      & 0.77       & 106        & 172      & 23.7\%   					& 10       & 29.4\% 							& 1.12       & 106        & 122      & 16.8\%							& 9        & 26.5\% 							\\
3      & 0.06       & 90         & 40       & 24.8\%   					& 16       & \hlc[OK]{61.5\%} 		            & 0.11       & 90         & 34       & 21.1\%							& 15       & \hlc[OK]{57.7\%} 		\\
4      & 3.20       & 96         & 63       & 13.7\%   					& 0        & \hlc[KO]{0.0\%}  		            & 1.24       & 94         & 30       & 6.5\%							& 0        & \hlc[KO]{0.0\%}  		\\
5      & 3.56       & 89         & 142      & \hlc[OK]{35.9\%}		& 4        & 12.5\% 							    & 5.27       & 89         & 12       & \hlc[KO]{3.0\%}		& 4        & 12.5\% 							\\
6      & 0.04       & 88         & 0        & \hlc[KO]{0.0\%}  	& 0        & \hlc[KO]{0.0\%}  		                    & 0.06       & 89         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
7      & 208.20     & 108        & 125      & 21.4\%   					& 0        & \hlc[KO]{0.0\%}  		            & 293.78     & 108        & 2        & \hlc[KO]{0.3\%}		& 0        & \hlc[KO]{0.0\%}  		\\
8      & 0.13       & 88         & 8        & 21.1\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.04       & 88         & 6        & 15.8\%							& 0        & \hlc[KO]{0.0\%}  		\\
9      & 12.25      & 121        & 317      & \hlc[OK]{53.0\%} 	& 15       & 30.0\% 							        & 18.10      & 121        & 215      & \hlc[OK]{36.0\%}		& 11       & 22.0\% 							\\
10     & 2.43       & 111        & 390      & \hlc[OK]{41.9\%} 	& 20       & \hlc[OK]{47.6\%} 		                    & 1.96       & 110        & 230      & 24.7\%							& 17       & \hlc[OK]{40.5\%} 		\\
11     & 0.00       & 51         & 0        & N/A      					& 0        & N/A    							& 0.00       & 51         & 0        & N/A								& 0        & N/A    							\\
12     & 574.35     & 329        & 1648     & \hlc[OK]{52.5\%}   & 27       & \hlc[OK]{38.0\%}			                & 293.97     & 284        & 1374     & \hlc[OK]{43.7\%}		& 20       & 28.2\% 							\\
13     & 17.54      & 140        & 159      & 18.4\%   					& 3        & 9.1\% 								& 2.53       & 115        & 36       & \hlc[KO]{4.2\%}		& 2        & 6.1\% 								\\
14     & 0.10       & 82         & 16       & 32.0\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.13       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
15     & 6.15       & 101        & 108      & 29.4\%   					& 2        & 22.2\% 							& 8.64       & 101        & 75       & 20.4\%							& 2        & 22.2\% 							\\
16     & 0.02       & 76         & 0        & \hlc[KO]{0.0\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.02       & 76         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
17     & 10.18      & 119        & 706      & \hlc[OK]{49.3\%}   & 13       & 26.5\% 							        & 11.31      & 119        & 533      & \hlc[OK]{37.2\%}		& 10       & 20.4\% 							\\
18     & 0.22       & 96         & 18       & 9.6\%    					& 1        & \hlc[KO]{4.8\%} 			        & 0.32       & 96         & 18       & 9.6\%							& 1        & \hlc[KO]{4.8\%} 			\\
19     & 0.05       & 83         & 2        & 13.3\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.08       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
20     & 0.17       & 88         & 41       & \hlc[OK]{38.7\%}		& 5        & \hlc[OK]{62.5\%}			            & 0.14       & 88         & 37       & 34.9\%							& 5        & \hlc[OK]{62.5\%} 		\\
21     & 0.03       & 76         & 16       & 20.8\%   					& 3        & \hlc[OK]{42.9\%}			        & 0.06       & 76         & 14       & 18.2\%							& 3        & \hlc[OK]{42.9\%} 		\\
22     & 0.03       & 75         & 6        & 26.1\%   					& 1        & 8.3\% 	 	 						& 0.08       & 75         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
23     & 0.78       & 99         & 30       & 5.8\%    					& 0        & \hlc[KO]{0.0\%}  		            & 0.84       & 98         & 8        & \hlc[KO]{1.5\%}		& 0        & \hlc[KO]{0.0\%}  		\\
24     & 150.15     & 177        & 843      & 23.4\%   					& 26       & 29.2\% 							& 52.22      & 159        & 586      & 16.3\%							& 22       & 24.7\% 							\\
25     & 0.41       & 78         & 2        & \hlc[KO]{4.7\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.06       & 76         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
26     & 22.69      & 157        & 229      & 13.2\%   					& 11       & 15.1\% 							& 13.46      & 138        & 138      & 8.0\%							& 11       & 15.1\% 							\\
27     & 21.76      & 160        & 174      & 24.9\%   					& 8        & 30.8\% 							& 5.22       & 122        & 145      & 20.7\%							& 6        & 23.1\% 							\\
28     & 0.32       & 95         & 27       & 15.5\%   					& 5        & 14.3\% 							& 0.17       & 94         & 17       & 9.8\%							& 5        & 14.3\% 							\\
29     & 0.03       & 83         & 4        & 13.8\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.04       & 82         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
30     & 0.88       & 90         & 113      & 31.1\%   					& 8        & 22.9\% 							& 0.60       & 90         & 32       & 8.8\%							& 4        & 11.4\% 							\\
31     & 0.00       & 58         & 0        & \hlc[KO]{0.0\%}    & 0        & N/A    							        & 0.00       & 58         & 0        & \hlc[KO]{0.0\%}		& 0        & N/A    							\\
32     & 53.28      & 139        & 1496     & \hlc[OK]{57.9\%}   & 10       & 21.3\%								    & 48.28      & 139        & 1432     & \hlc[OK]{55.4\%}		& 5        & 10.6\% 							\\
33     & 0.95       & 94         & 48       & 13.7\%   					& 1        & 8.3\%								& 0.36       & 94         & 10       & \hlc[KO]{2.9\%}		& 1        & 8.3\% 								\\
34     & 0.38       & 90         & 8        & 9.2\%    					& 1        & 7.1\%								& 0.11       & 88         & 2        & \hlc[KO]{2.3\%}		& 1        & 7.1\% 								\\
35     & 170.80     & 108        & 536      & \hlc[OK]{46.9\%}   & 43       & 26.2\%								    & 236.64     & 107        & 402      & \hlc[OK]{35.2\%}		& 34       & 20.7\% 							\\
36     & 0.22       & 98         & 28       & 21.2\%   					& 3        & 15.8\%								& 0.25       & 98         & 20       & 15.2\%							& 2        & 10.5\% 							\\
37     & 0.03       & 82         & 8        & 21.1\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.08       & 82         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
38     & 6.64       & 329        & 196      & 10.8\%   					& 7        & 17.9\%								& 6.46       & 329        & 87       & \hlc[KO]{4.8\%}		& 7        & 17.9\% 							\\
39     & 9.64       & 102        & 186      & 26.8\%   					& 14       & \hlc[OK]{41.2\%}			        & 11.11      & 101        & 106      & 15.3\%							& 13       & \hlc[OK]{38.2\%}			\\
40     & 123.95     & 139        & 486      & 31.2\%   					& 19       & 31.7\%								& 172.47     & 139        & 233      & 15.0\%							& 14       & 23.3\% 							\\
41     & 0.88       & 110        & 8        & \hlc[KO]{2.2\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.35       & 108        & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
42     & 26.16      & 110        & 826      & \hlc[OK]{37.0\%}		& 27       & 22.1\%								    & 12.24      & 109        & 659      & 29.5\%							& 20       & 16.4\% 							\\
43     & 14.52      & 158        & 741      & 32.0\%   					& 37       & 29.4\%								& 7.69       & 158        & 593      & 25.6\%							& 30       & 23.8\% 							\\
44     & 0.04       & 84         & 0        & \hlc[KO]{0.0\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.01       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
45     & 521.35     & 253        & 445      & 11.5\%   					& 24       & 16.0\%								& 11.14      & 251        & 254      & 6.6\%							& 16       & 10.7\% 							\\
46     & 469.72     & 350        & 1097     & 22.4\%   					& 34       & 17.3\%								& 146.85     & 350        & 750      & 15.3\%							& 26       & 13.3\% 							\\
47     & 9965.49    & 1458       & 14356    & 32.8\%   					& 388      & 26.3\%								& 9065.11    & 1458       & 9196     & 21.0\%							& 293      & 19.9\% 							\\
48     & 234.72     & 413        & 427      & 9.6\%    					& 18       & 16.7\%								& 22.23      & 400        & 222      & 5.0\%							& 14       & 13.0\% 							\\
49     & 0.24       & 142        & 6        & \hlc[KO]{1.7\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.33       & 142        & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
50     & 8.37       & 116        & 234      & 11.2\%   					& 1        & \hlc[KO]{1.5\%}  		            & 3.55       & 111        & 179      & 8.5\%							& 1        & \hlc[KO]{1.5\%}			\\
51     & 32.61      & 172        & 291      & 11.2\%   					& 16       & 14.5\%								& 13.10      & 172        & 91       & \hlc[KO]{3.5\%}		& 10       & 9.1\% 								\\
52     & 2430.47    & 602        & 1385     & \hlc[OK]{39.0\%}		& 56       & 26.4\%								    & 1241.06    & 601        & 1034     & 29.2\%							& 48       & 22.6\% 							\\
53     & 197.16     & 376        & 1293     & 17.8\%   					& 55       & 23.6\%								& 87.11      & 375        & 689      & 9.5\%							& 42       & 18.0\% 							\\
54     & 801.49     & 310        & 227      & 8.4\%    					& 11       & 15.3\%								& 722.07     & 261        & 112      & \hlc[KO]{4.1\%}		& 7        & 9.7\% 								\\
55     & 36.18      & 292        & 240      & 7.8\%    					& 5        & \hlc[KO]{4.3\%}  		            & 10.73      & 275        & 47       & \hlc[KO]{1.5\%}		& 5        & 4.3\% 								\\
56     & 655.46     & 1403       & 58       & 14.9\%   					& 5        & 20.8\%								& 0.67       & 176        & 38       & 9.8\%							& 4        & 16.7\% 							\\
57     & 617.86     & 352        & 1245     & 17.4\%   					& 36       & 7.4\%								& 79.75      & 202        & 796      & 11.1\%							& 26       & 5.4\% 								\\
58     & 0.19       & 95         & 2        & \hlc[KO]{1.2\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.09       & 95         & 2        & \hlc[KO]{1.2\%}		& 0        & \hlc[KO]{0.0\%}  		\\
59     & 2.80       & 211        & 29       & \hlc[OK]{39.2\%}		& 3        & \hlc[OK]{42.9\%}			            & 0.09       & 191        & 16       & 21.6\%							& 1        & 14.3\% 							\\
60     & 13764.80   & 854        & 15570    & \hlc[OK]{52.6\%}   & 176      & 16.8\%								    & 5467.20    & 781        & 10465    & \hlc[OK]{35.4\%}		& 90       & 8.6\% 								\\
61     & 6594.13    & 1317       & 21034    & \hlc[OK]{38.3\%}		& 256      & 15.3\%								    & 4312.97    & 873        & 10891    & 19.8\%							& 206      & 12.3\% 							\\
62     & 1022.12    & 1075       & 5833     & 22.5\%   					& 127      & 19.8\%								& 471.98     & 1074       & 3698     & 14.3\%							& 97       & 15.2\% 							\\
63     & 19738.40   & 2635       & 16947    & \hlc[OK]{52.7\%}   & 231      & 28.0\%								    & 12533.30   & 2642       & 12309    & \hlc[OK]{38.3\%}		& 159      & 19.2\% 							\\
64     & 114.66     & 380        & 176      & 9.8\%    					& 11       & 17.7\%								& 71.98      & 367        & 56       & \hlc[KO]{3.1\%}		& 5        & 8.1\% 								\\
65     & 1155.87    & 2716       & 1783     & 16.8\%   					& 61       & 18.5\%								& 132.82     & 325        & 1148     & 10.8\%							& 51       & 15.5\% 							\\
        % \hline

   \end{longtable} 
}





==> tables/results-with-decimal.tex <==
{
% \begin{landscape}
    \rowcolors{2}{gray!10}{white}
	\scriptsize % \tiny % \footnotesize
    \begin{longtable}{
            % @{\extracolsep{\fill}}
            >{\raggedright\arraybackslash}m{1.5cm}
            >{\centering\arraybackslash}m{0.35cm}
            >{\centering\arraybackslash}m{0.35cm} |
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.75cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.8cm} ||
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.75cm}
            >{\centering\arraybackslash}m{0.6cm}
            >{\centering\arraybackslash}m{0.8cm}
    }
        \toprule
        \rowcolor{white}
        \multicolumn{3}{c}{} & \multicolumn{6}{c}{\textbf{Threshold 90\%}} & \multicolumn{6}{c}{\textbf{Threshold 99\%}}\\
          & \textbf{Fn}s & \textbf{Tr}s & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} \\
		\midrule
		\endfirsthead

		\toprule
        \rowcolor{white}
        \multicolumn{3}{c}{} & \multicolumn{6}{c}{\textbf{Threshold 90\%}} & \multicolumn{6}{c}{\textbf{Threshold 99\%}}\\
          & \textbf{Fn}s & \textbf{Tr}s & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} & \textbf{Time} & \textbf{Mem} & \textbf{\#Fn} & \textbf{\%Fn} & \textbf{\#Tr} & \textbf{\%Tr} \\
		\midrule
		\endhead


		\midrule
        \rowcolor{white}
		\multicolumn{13}{r}{\textit{Continued on next page}} \\
		\midrule
		\endfoot

		\bottomrule
        \rowcolor{white}
        \multicolumn{13}{c}{ } \\
        \caption{TODO}
        \label{tab:results}
		\endlastfoot

\href{https://github.com/dtolnay/syn}{syn}                                    & 11140    & 129    & 167.12     & 200        & 2394     & 21.5\%   					& 36       & 27.9\% 							& 200.97     & 181        & 1313     & 11.8\%							& 30       & 23.3\% 							\\
\href{https://github.com/rust-lang/hashbrown}{hashbrown}                      & 727      & 34     & 0.77       & 106        & 172      & 23.7\%   					& 10       & 29.4\% 							& 1.12       & 106        & 122      & 16.8\%							& 9        & 26.5\% 							\\
\href{https://github.com/bitflags/bitflags}{bitflags}                         & 161      & 26     & 0.06       & 90         & 40       & 24.8\%   					& 16       & \hlc[OK]{61.5\%} 		            & 0.11       & 90         & 34       & 21.1\%							& 15       & \hlc[OK]{57.7\%} 		\\
\href{https://github.com/dtolnay/proc-macro2}{proc-macro2}                    & 460      & 16     & 3.20       & 96         & 63       & 13.7\%   					& 0        & \hlc[KO]{0.0\%}  		            & 1.24       & 94         & 30       & 6.5\%							& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/dtolnay/quote}{quote}                                & 395      & 32     & 3.56       & 89         & 142      & \hlc[OK]{35.9\%}		& 4        & 12.5\% 							    & 5.27       & 89         & 12       & \hlc[KO]{3.0\%}		& 4        & 12.5\% 							\\
\href{https://github.com/marshallpierce/rust-base64}{base64}                  & 84       & 14     & 0.04       & 88         & 0        & \hlc[KO]{0.0\%}  	& 0        & \hlc[KO]{0.0\%}  		                    & 0.06       & 89         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/rust-lang/libc}{libc}                                & 583      & 10     & 208.20     & 108        & 125      & 21.4\%   					& 0        & \hlc[KO]{0.0\%}  		            & 293.78     & 108        & 2        & \hlc[KO]{0.3\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/rust-random/getrandom}{getrandom}                    & 38       & 3      & 0.13       & 88         & 8        & 21.1\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.04       & 88         & 6        & 15.8\%							& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/rust-random/rand}{rand}                              & 598      & 50     & 12.25      & 121        & 317      & \hlc[OK]{53.0\%} 	& 15       & 30.0\% 							        & 18.10      & 121        & 215      & \hlc[OK]{36.0\%}		& 11       & 22.0\% 							\\
\href{https://github.com/indexmap-rs/indexmap}{indexmap}                      & 931      & 42     & 2.43       & 111        & 390      & \hlc[OK]{41.9\%} 	& 20       & \hlc[OK]{47.6\%} 		                    & 1.96       & 110        & 230      & 24.7\%							& 17       & \hlc[OK]{40.5\%} 		\\
\href{https://github.com/rust-lang/cfg-if}{cfg-if}                            & 0        & 0      & 0.00       & 51         & 0        & N/A      					& 0        & N/A    							& 0.00       & 51         & 0        & N/A								& 0        & N/A    							\\
\href{https://github.com/serde-rs/serde}{serde}                               & 3141     & 71     & 574.35     & 329        & 1648     & \hlc[OK]{52.5\%}   & 27       & \hlc[OK]{38.0\%}			                & 293.97     & 284        & 1374     & \hlc[OK]{43.7\%}		& 20       & 28.2\% 							\\
\href{https://github.com/rust-itertools/itertools}{itertools}                 & 865      & 33     & 17.54      & 140        & 159      & 18.4\%   					& 3        & 9.1\% 								& 2.53       & 115        & 36       & \hlc[KO]{4.2\%}		& 2        & 6.1\% 								\\
\href{https://github.com/cuviper/autocfg}{autocfg}                            & 50       & 2      & 0.10       & 82         & 16       & 32.0\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.13       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/BurntSushi/memchr}{memchr}                           & 367      & 9      & 6.15       & 101        & 108      & 29.4\%   					& 2        & 22.2\% 							& 8.64       & 101        & 75       & 20.4\%							& 2        & 22.2\% 							\\
\href{https://github.com/dtolnay/itoa}{itoa}                                  & 18       & 3      & 0.02       & 76         & 0        & \hlc[KO]{0.0\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.02       & 76         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/serde-rs/json}{json}                                 & 1432     & 49     & 10.18      & 119        & 706      & \hlc[OK]{49.3\%}   & 13       & 26.5\% 							        & 11.31      & 119        & 533      & \hlc[OK]{37.2\%}		& 10       & 20.4\% 							\\
\href{https://github.com/dtolnay/thiserror}{thiserror}                        & 188      & 21     & 0.22       & 96         & 18       & 9.6\%    					& 1        & \hlc[KO]{4.8\%} 			        & 0.32       & 96         & 18       & 9.6\%							& 1        & \hlc[KO]{4.8\%} 			\\
\href{https://github.com/dtolnay/unicode-ident}{unicode-ident}                & 15       & 1      & 0.05       & 83         & 2        & 13.3\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.08       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/matklad/once_cell}{once\_cell}                       & 106      & 8      & 0.17       & 88         & 41       & \hlc[OK]{38.7\%}		& 5        & \hlc[OK]{62.5\%}			            & 0.14       & 88         & 37       & 34.9\%							& 5        & \hlc[OK]{62.5\%} 		\\
\href{https://github.com/rust-lang/log}{log}                                  & 77       & 7      & 0.03       & 76         & 16       & 20.8\%   					& 3        & \hlc[OK]{42.9\%}			        & 0.06       & 76         & 14       & 18.2\%							& 3        & \hlc[OK]{42.9\%} 		\\
\href{https://github.com/withoutboats/heck}{heck}                             & 23       & 12     & 0.03       & 75         & 6        & 26.1\%   					& 1        & 8.3\% 	 	 						& 0.08       & 75         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/rust-lang/cc-rs}{cc}                                 & 517      & 20     & 0.78       & 99         & 30       & 5.8\%    					& 0        & \hlc[KO]{0.0\%}  		            & 0.84       & 98         & 8        & \hlc[KO]{1.5\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/rust-lang/regex}{regex}                              & 3597     & 89     & 150.15     & 177        & 843      & 23.4\%   					& 26       & 29.2\% 							& 52.22      & 159        & 586      & 16.3\%							& 22       & 24.7\% 							\\
\href{https://github.com/dtolnay/ryu}{ryu}                                    & 43       & 3      & 0.41       & 78         & 2        & \hlc[KO]{4.7\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.06       & 76         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/clap-rs/clap}{clap}                                  & 1730     & 73     & 22.69      & 157        & 229      & 13.2\%   					& 11       & 15.1\% 							& 13.46      & 138        & 138      & 8.0\%							& 11       & 15.1\% 							\\
\href{https://github.com/aho-corasick}{aho-corasick}                          & 699      & 26     & 21.76      & 160        & 174      & 24.9\%   					& 8        & 30.8\% 							& 5.22       & 122        & 145      & 20.7\%							& 6        & 23.1\% 							\\
\href{https://github.com/servo/rust-smallvec}{smallvec}                       & 174      & 35     & 0.32       & 95         & 27       & 15.5\%   					& 5        & 14.3\% 							& 0.17       & 94         & 17       & 9.8\%							& 5        & 14.3\% 							\\
\href{https://github.com/rapidfuzz/strsim-rs}{strsim}                         & 29       & 3      & 0.03       & 83         & 4        & 13.8\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.04       & 82         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/Amanieu/parking_lot}{parking\_lot}                   & 363      & 35     & 0.88       & 90         & 113      & 31.1\%   					& 8        & 22.9\% 							& 0.60       & 90         & 32       & 8.8\%							& 4        & 11.4\% 							\\
\href{https://github.com/rust-lang-nursery/lazy-static.rs}{lazy\_static}      & 2        & 0      & 0.00       & 58         & 0        & \hlc[KO]{0.0\%}    & 0        & N/A    							        & 0.00       & 58         & 0        & \hlc[KO]{0.0\%}		& 0        & N/A    							\\
\href{https://github.com/rust-num/num-traits}{num-traits}                     & 2585     & 47     & 53.28      & 139        & 1496     & \hlc[OK]{57.9\%}   & 10       & 21.3\%								    & 48.28      & 139        & 1432     & \hlc[OK]{55.4\%}		& 5        & 10.6\% 							\\
\href{https://github.com/rust-lang/socket2}{socket2}                          & 350      & 12     & 0.95       & 94         & 48       & 13.7\%   					& 1        & 8.3\%								& 0.36       & 94         & 10       & \hlc[KO]{2.9\%}		& 1        & 8.3\% 								\\
\href{https://github.com/dtolnay/semver}{semver}                              & 87       & 14     & 0.38       & 90         & 8        & 9.2\%    					& 1        & 7.1\%								& 0.11       & 88         & 2        & \hlc[KO]{2.3\%}		& 1        & 7.1\% 								\\
\href{https://github.com/RustCrypto/traits}{digest}                           & 1142     & 164    & 170.80     & 108        & 536      & \hlc[OK]{46.9\%}   & 43       & 26.2\%								    & 236.64     & 107        & 402      & \hlc[OK]{35.2\%}		& 34       & 20.7\% 							\\
\href{https://github.com/rayon-rs/either}{either}                             & 132      & 19     & 0.22       & 98         & 28       & 21.2\%   					& 3        & 15.8\%								& 0.25       & 98         & 20       & 15.2\%							& 2        & 10.5\% 							\\
\href{https://github.com/SergioBenitez/version_check}{version\_check}         & 38       & 2      & 0.03       & 82         & 8        & 21.1\%   					& 0        & \hlc[KO]{0.0\%}  		            & 0.08       & 82         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/bytecodealliance/rustix}{rustix}                     & 1809     & 39     & 6.64       & 329        & 196      & 10.8\%   					& 7        & 17.9\%								& 6.46       & 329        & 87       & \hlc[KO]{4.8\%}		& 7        & 17.9\% 							\\
\href{https://github.com/tokio-rs/bytes}{bytes}                               & 695      & 34     & 9.64       & 102        & 186      & 26.8\%   					& 14       & \hlc[OK]{41.2\%}			        & 11.11      & 101        & 106      & 15.3\%							& 13       & \hlc[OK]{38.2\%}			\\
\href{https://github.com/time-rs/time}{time}                                  & 1558     & 60     & 123.95     & 139        & 486      & 31.2\%   					& 19       & 31.7\%								& 172.47     & 139        & 233      & 15.0\%							& 14       & 23.3\% 							\\
\href{https://github.com/servo/rust-url}{url}                                 & 365      & 34     & 0.88       & 110        & 8        & \hlc[KO]{2.2\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.35       & 108        & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/toml-rs/toml}{toml}                                  & 2233     & 122    & 26.16      & 110        & 826      & \hlc[OK]{37.0\%}		& 27       & 22.1\%								    & 12.24      & 109        & 659      & 29.5\%							& 20       & 16.4\% 							\\
\href{https://github.com/rust-lang/futures-rs}{futures}                       & 2313     & 126    & 14.52      & 158        & 741      & 32.0\%   					& 37       & 29.4\%								& 7.69       & 158        & 593      & 25.6\%							& 30       & 23.8\% 							\\
\href{https://github.com/rust-lang/glob}{glob}                                & 32       & 7      & 0.04       & 84         & 0        & \hlc[KO]{0.0\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.01       & 83         & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/quickwit-oss/tantivy}{tantivy}                       & 3871     & 150    & 521.35     & 253        & 445      & 11.5\%   					& 24       & 16.0\%								& 11.14      & 251        & 254      & 6.6\%							& 16       & 10.7\% 							\\
\href{https://github.com/tauri-apps/tauri}{tauri}                             & 4898     & 196    & 469.72     & 350        & 1097     & 22.4\%   					& 34       & 17.3\%								& 146.85     & 350        & 750      & 15.3\%							& 26       & 13.3\% 							\\
\href{https://github.com/pola-rs/polars}{polars}                              & 43805    & 1476   & 9965.49    & 1458       & 14356    & 32.8\%   					& 388      & 26.3\%								& 9065.11    & 1458       & 9196     & 21.0\%							& 293      & 19.9\% 							\\
\href{https://github.com/rust-lang/cargo}{cargo}                              & 4441     & 108    & 234.72     & 413        & 427      & 9.6\%    					& 18       & 16.7\%								& 22.23      & 400        & 222      & 5.0\%							& 14       & 13.0\% 							\\
\href{https://github.com/sharkdp/bat}{bat}                                    & 356      & 16     & 0.24       & 142        & 6        & \hlc[KO]{1.7\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.33       & 142        & 0        & \hlc[KO]{0.0\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/BurntSushi/ripgrep}{ripgrep}                         & 2096     & 66     & 8.37       & 116        & 234      & 11.2\%   					& 1        & \hlc[KO]{1.5\%}  		            & 3.55       & 111        & 179      & 8.5\%							& 1        & \hlc[KO]{1.5\%}			\\
\href{https://github.com/cloudflare/quiche}{quiche}                           & 2607     & 110    & 32.61      & 172        & 291      & 11.2\%   					& 16       & 14.5\%								& 13.10      & 172        & 91       & \hlc[KO]{3.5\%}		& 10       & 9.1\% 								\\
\href{https://github.com/influxdata/influxdb}{influxdb}                       & 3547     & 212    & 2430.47    & 602        & 1385     & \hlc[OK]{39.0\%}		& 56       & 26.4\%								    & 1241.06    & 601        & 1034     & 29.2\%							& 48       & 22.6\% 							\\
\href{https://github.com/typst/typst}{typst}                                  & 7260     & 233    & 197.16     & 376        & 1293     & 17.8\%   					& 55       & 23.6\%								& 87.11      & 375        & 689      & 9.5\%							& 42       & 18.0\% 							\\
\href{https://github.com/alacritty/alacritty}{alacritty}                      & 2710     & 72     & 801.49     & 310        & 227      & 8.4\%    					& 11       & 15.3\%								& 722.07     & 261        & 112      & \hlc[KO]{4.1\%}		& 7        & 9.7\% 								\\
\href{https://github.com/helix-editor/helix}{helix}                           & 3080     & 116    & 36.18      & 292        & 240      & 7.8\%    					& 5        & \hlc[KO]{4.3\%}  		            & 10.73      & 275        & 47       & \hlc[KO]{1.5\%}		& 5        & 4.3\% 								\\
\href{https://github.com/Nukesor/pueue}{pueue}                                & 389      & 24     & 655.46     & 1403       & 58       & 14.9\%   					& 5        & 20.8\%								& 0.67       & 176        & 38       & 9.8\%							& 4        & 16.7\% 							\\
\href{https://github.com/GitoxideLabs/gitoxide}{gitoxide}                     & 7148     & 484    & 617.86     & 352        & 1245     & 17.4\%   					& 36       & 7.4\%								& 79.75      & 202        & 796      & 11.1\%							& 26       & 5.4\% 								\\
\href{https://github.com/EmbarkStudios/texture-synthesis}{texture-synthesis}  & 166      & 10     & 0.19       & 95         & 2        & \hlc[KO]{1.2\%}    & 0        & \hlc[KO]{0.0\%}  		                    & 0.09       & 95         & 2        & \hlc[KO]{1.2\%}		& 0        & \hlc[KO]{0.0\%}  		\\
\href{https://github.com/n0-computer/sendme}{sendme}                          & 74       & 7      & 2.80       & 211        & 29       & \hlc[OK]{39.2\%}		& 3        & \hlc[OK]{42.9\%}			            & 0.09       & 191        & 16       & 21.6\%							& 1        & 14.3\% 							\\
\href{https://github.com/unionlabs/union}{union}                              & 29581    & 1050   & 13764.80   & 854        & 15570    & \hlc[OK]{52.6\%}   & 176      & 16.8\%								    & 5467.20    & 781        & 10465    & \hlc[OK]{35.4\%}		& 90       & 8.6\% 								\\
\href{https://github.com/zed-industries/zed}{zed}                             & 54980    & 1674   & 6594.13    & 1317       & 21034    & \hlc[OK]{38.3\%}		& 256      & 15.3\%								    & 4312.97    & 873        & 10891    & 19.8\%							& 206      & 12.3\% 							\\
\href{https://github.com/charliermarsh/ruff}{ruff}                            & 25887    & 640    & 1022.12    & 1075       & 5833     & 22.5\%   					& 127      & 19.8\%								& 471.98     & 1074       & 3698     & 14.3\%							& 97       & 15.2\% 							\\
\href{https://github.com/juspay/hyperswitch}{hyperswitch}                     & 32172    & 826    & 19738.40   & 2635       & 16947    & \hlc[OK]{52.7\%}   & 231      & 28.0\%								    & 12533.30   & 2642       & 12309    & \hlc[OK]{38.3\%}		& 159      & 19.2\% 							\\
\href{https://github.com/lapce/lapce}{lapce}                                  & 1797     & 62     & 114.66     & 380        & 176      & 9.8\%    					& 11       & 17.7\%								& 71.98      & 367        & 56       & \hlc[KO]{3.1\%}		& 5        & 8.1\% 								\\
\href{https://github.com/nushell/nushell}{nushell}                            & 10592    & 330    & 1155.87    & 2716       & 1783     & 16.8\%   					& 61       & 18.5\%								& 132.82     & 325        & 1148     & 10.8\%							& 51       & 15.5\% 							\\
       % \hline

   \end{longtable}
}

